Adaptive Task Planning for Large-Scale Robotized Warehouses

Robotized warehouses are deployed to automatically distribute millions of items brought by the massive logistic orders from e-commerce. A key to automated item distribution is to plan paths for robots, also known as task planning, where each task is to deliver racks with items to pickers for processing and then return the rack back. Prior solutions are unfit for large-scale robotized warehouses due to the inflexibility to time-varying item arrivals and the low efficiency for high throughput. In this paper, we propose a new task planning problem called TPRW, which aims to minimize the end-to-end makespan that incorporates the entire item distribution pipeline, known as a fulfilment cycle. Direct extensions from state-of-the-art path finding methods are ineffective to solve the TPRW problem because they fail to adapt to the bottleneck variations of fulfillment cycles. In response, we propose Efficient Adaptive Task Planning, a framework for large-scale robotized warehouses with time-varying item arrivals. It adaptively selects racks to fulfill at each timestamp via reinforcement learning, accounting for the time-varying bottleneck of the fulfillment cycles. Then it finds paths for robots to transport the selected racks. The framework adopts a series of efficient optimizations on both time and memory to handle large-scale item throughput. Evaluations on both synthesized and real data show an improvement of $37.1\%$ in effectiveness and $75.5\%$ in efficiency over the state-of-the-arts.

==> body/trash.tex <==

Based on the above analysis, we notice that the reason why greedy method may trap into bad solutions can be explained intuitively as follows.
\begin{itemize}
    \item Lack the consideration of the trade-off between deliver frequency and waiting time.
    Instead of delivering a rack as soon as task emerges, waiting some time some more tasks may emerge and thus we can reduce the times of moving back-and-forth. 
    \item Lack the consideration of the future. 
    The greedy method only assign AMR to those tasks whose picker is most slack currently.
    But we should also considering the remaining picking tasks of the picker.
\end{itemize}

To overcome these issues, we propose reinforcement learning based method, as we will introduce next.


% f_r = \left\{
% \begin{array}{rcl}
% d(l_a, l_r) + d(l_r, l_{p_r}) + d(l_{p_r}, l_r) + \xi_o& & \text{if } k = 1 \\
% \max_{o'\in \tau_r^{(t')}}\{F(o'), t + d(l^{(t)}_a, l_{r}) \\
% + d(l_{r}, l_{p_{r}})\} + \xi_o + d(l_{r}, l_{p_{r}}) & & \text{else}
% \end{array} \right.
    
where $t$ is the time the assignment is made, $t'$ is the time the task delivered to the picker, $a$ is the assigned AMR, $r$ and $p$ is the corresponding rack and picker, respectively.
$d(\cdot, \cdot)$ denotes the distance (such as Manhattan or Eculidean distance) between two locations.
By assuming the moving speed is unit distance per unit time, its value is same as time usage.
Intuitively, if there is no rack in queue of the picker, the finish time of the task is the summation of shipping(picking-up, delivering and returning) and picking time.
Otherwise, the time will be the summation of heading to the picker and/or queuing (\ie the maximize term), piking and returning.

\begin{definition}[Task]
A task $o$ can be denoted as $\langle ts_o, \xi_o, r_o \rangle$, wherein $ts_o$ is the emerging time of task $o$, $\xi_o$ is the estimated picking time usage of task $o$ and $r_o$ is the rack to which the task belongs.
\end{definition}
Task arrives following an online manner.
$\xi_o$ is usually between $20$\textasciitilde$40$ seconds.
We use $O$ to denote all available tasks (\ie tasks have not been fulfilled).
Each task has a corresponding rack, as we will introduce below.

$ts_o, \xi_o, r_o$ & \makecell[l]{emerging time, picking time, corresponding \\ rack of task $o$} \\

\subsection{Problem Analysis}
\label{subsec:hardness}
In this subsection, we analysis the hardness of RTAP.
This problem is really hard to get to the optimal solution mainly because the following two reasons.
\textit{(i)} Tasks arrive dynamically and the online setting makes it difficult to get the optimal solution.
\textit{(ii)} Even without the online setting, the offline version of RTAP is still NP-Hard.

To prove this, we first formerly define the offline version of RTAP, then we reduce the classic NP-Complete problem Traveling Salesman Problem (TSP) to RTAP to prove its NP-Hardness.
Since it is offline, all the tasks are known at first, and we can accumulate tasks at the same rack and view them as one task.
In that case we can omit the racks and the emerging time of each task and replace task with located task.
A located task has an extra location property $l_o$ than original task which has the same value as its corresponding rack location, so it can be denoted as $\langle \xi_o, l_o, \rangle$ representing it's estimated picking time and the location of it's corresponding rack.

\begin{definition}[offline-RTAP]
Given a set of robots $A$, a set of pickers $P$ and a set of located tasks $O_l$, the designed algorithm $\mathcal{A}$ is required to provide a series of assignment schemes $\{S_1, ..., S_k\}$ and routing schemes $\{U_1, ..., U_k\}$, such that
\begin{equation}
\begin{aligned}
    & \min M \\
    & S_i \text{ is feasible }\forall 1 \le i \le k  \\
    & \{S_i|\forall 1 \le i \le k\}  \text{ is sufficient} \\
    & \{U_i|\forall 1 \le i \le k \} \text{ is conflict-free}
    \nonumber
\end{aligned}
\end{equation}
\end{definition}
Next we show how to convert a TSP problem instance into an offline-RTAP problem.
\begin{theorem}
	offline-RTAP is NP-Hard.
\end{theorem}
\begin{proof}
A TSP instance contains an undirected weighted graph $G = \langle V, E \rangle$, and the optimization goal is to find a shortest path $P$ that minimizes $\sum_{(u, v)\in P} e(u, v)$ that contains all vertices once and only once.
W.l.o.g., we assuming the edge weight satisfying triangle inequality, \ie $\forall u, v, w \in V, e(u,w) + e(w, v) \le e(u, v)$.
This assumption does not change the NP-completeness property of TSP\cite{IPL00Bock}.

We build an offline-RTAP instance based on a TSP instance as follows.
First, we set one robot and $|V|$ located tasks, whose picking time is zero.
Then we set all locations of tasks satisfying the distance equals the edge weight in original graph $G$.
This can be done in polynomial time by solving the equation set.
At last we set $|V|$ pickers for each task and set the picker's location the same as that of task.
Since there is only one robot, finding the routing scheme can be simply calculated by breadth first search, so we mainly consider the calculation of assignment.
To generate a series assignment with single AMR without considering picking time is equivalent to finding a path which visits all racks once and only once.
If we can solve the above offline-RTAP instance in polynomial time, we can find a optimal solution for TSP.
So offline-RTAP is NP-hard.
% We will find assignment schemes $\{S_1, S_2, ...S_n\}$ that minimize the $\max F(o)$.
% Since each picker has only one task, so for each task $o$ and we have set $\xi_o$ to be 0, we have
% $F(o) = t + d(l^{(t)}_a, l_{o}) + 2 * d(l_{o}, l_{p_{r}})\forall o \in T$.
% Besides, since we have set the location of picker the same as task.
% So $d(l_{o}, l_{p_{r}}) = d(l_{o}, l_{o}) = 0$.
% Now we have 
% $F(o) = t + d(l^{(t)}_a, l_{o})\forall o \in T$.
% Since there is only one AMR, so each scheme contains only one task, so we can sort the tasks based on the assigned order by $o_1, o_2, ..., o_{|T|}$ and $\max F(o) = F(o_{|T|})$.
% So $F(o_{|T|}) = t + d(l^{(t)}_a, l_{o})$, where $t$ is the assignment time.
% if $F(o_{|T|})$ is minimized, then $t$ is the time right after $o_{|T| - 1}$ is finished, otherwise we can bring forward to that moment and the total makespan will be reduced.
% At time $t$, the AMR has just returned the last task, so $l^{(t)}_a=l_{o_{|T|-1}}$.
% Recursively, we have
% \begin{equation}
% \begin{aligned}
%     \max F(o) & = F(o_{|T|}) = t + d(l^{(t)}_a, l_{o_{|T|}}) \\
%     & = F(o_{|T| - 1}) + d(l_{o_{|T|-1}}, l_{o_{|T|}}) = ... \\
%     & = d(l_{o_1}, l_{o_2}) + ... + d(l_{o_{|T|-1}}, l_{o_{|T|}}) \\
% \end{aligned}
% \end{equation}
% Based on the conversion, the distance between two tasks equals the weight of the corresponding edge.
% So $\min \max F(o) = \min \sum_{(u,v)\in P} e(u,v)$.
% In other words, if we can solve offline-ATAP in polynomial time, we can solve TSP in polynomial time, too.
\end{proof}

\fakeparagraph{Performance analysis}
The assignment part of Greedy method has the time complexity of $O(|P|\log |P| + |R| \cdot |A|)$.
As for the routing part, its complexity is $O(|S|\cdot M\cdot H\cdot W)$, where $H$ and $W$ denote the length and width of the warehouse and $M$ is the makespan.
% However, the algorithm suffers bad performance.
The Greedy algorithm suffers bad performance, in fact, it does not has a constant competitive ratio.
\begin{theorem}
	Greedy does not have a constant competitive ratio.
	The competitive ratio of Greedy is at least $O(k)$, where $k$ is the maximum number of tasks of one rack.
\end{theorem}

Based on efficient assignment in ABQL and conflict aware route query, the whole efficient-ABQL algorithm can be described in \algref{alg:eff-abql}.
\begin{algorithm}
\label{alg:eff-abql}
    \caption{Efficient-ABQL}
    \Input{$t$: the current time, $A$ available AMR set, $O$: task set, $\delta$: approximation parameter, $\beta$: learning rate, $\epsilon$: greedy parameter}
	\Output{$S, U$: assignment and routing scheme at time $t$}
	\If{$t = 0$}{
	    \text{build index, initialize q}
	}
	$S \leftarrow \text{ Efficient Assignment in ABQL}$ \\
	$U \leftarrow \emptyset$ \\
	\For{$\langle r, a \rangle \in S$}{
	    $u \leftarrow \text{ planing via Conflict-Aware Route Query}$ \\
	    $U \leftarrow U \cup u$ \\
	}
	\Return{$S, U$}
\end{algorithm}

We further reduce the time complexity by using $\epsilon$-greedy as a pruning trick.
Since there are only two actions, it is not easy that
So with $\frac{\epsilon}{2}$ probability we omit the following process and move on to consider next rack while the remaining $\frac{\epsilon}{2}$ probability we conduct normal $\epsilon$-greedy operation.

\fakeparagraph{AMR's Queuing Time (AQT)}
AMR's queuing time is defined as follows.
\begin{equation}
    AQT = \frac{1}{|A|} \sum_{a \in A}{\sum_{t}\mathbb{I}_{a \text{ is queuing at } t}}
\end{equation}
A smaller AQT indicates that the assignment algorithm will be aware of current picker's degree of business and try not to assign too many racks to a single picker.

There are two types of value function in reinforcement learning.
One is state value function $V(s)$ which maps the current state $s$ to the expected accumulated rewards while the other is action-state value function $q(s, \alpha)$ which maps the state-action pair to the expected accumulated rewards.
Deriving policy based on $q(s, \alpha)$ is usually simpler than that of $V(s)$, we only need to choose the $\arg\max_{\alpha'}q(s, \alpha')$ as the best action.

% Our problem is defined based on the automatic rack-to-picker scenario.
% As introduced in \secref{sec:intro}, robots ship racks from storage area to fixed located pickers back and forth.
% A complete fulfilling cycle contains five steps: picking-up, delivering, queuing, picking and returning (See \figref{fig:warehouse}).
% The scheduling is mainly about selecting suitable racks to deliver to pickers.
% It also includes planning paths for idle robots to fulfill the delivery task.
% The formal definitions of rack, picker and robot are as below.

% Each rack has a fixed corresponding picker due to some management requirements.
% For instance, a group of pickers and racks are arranged to serve orders (containing items stored on racks) from certain cities.
% The item set contains picking time of items which need picking.
% Items to be picked emerge dynamically when an online shopping user make orders.
% Different items has different picking time usages because of differences on size and weight.
% Each item's picking time consumption can be evaluated based on history data and it is input in our problem.
% We use $R$ to denote set of all racks.
% A good rack selection strategy largely depends on the dynamic character of item set $\tau_r$.
% It also requires consideration of the temporal status of pickers, as we will introduce next.

% When waiting to be picked, robots will carry the rack and queue in line.
% To avoid too much space usage, the queue usually confined in a narrow area thus no insertion or rearrangement is allowed, so the items are picked following ``first-come-first-serve'' rule.
% Intuitively, a bad rack selection policy will cause largely unbalanced queue lengths among pickers, while a good one will consider $e_p$ and $q_p$ to evaluate the picker's working status for better decision.
% We use $P$ to denote set of all pickers.

%After rack selection, we need planning paths for idle robots to fulfill the selected racks based on its location $l_a$ together with rack's location $l_r$ and picker's location $l_p$.

%It can be calculated as \equref{eq:finishPicker}, and the max term in \equref{eq:finishRack} denotes queuing time.

% The goal is to improve the picking efficiency of a smart warehouse. 
% To quantify this, we bring in \emph{makespan} (denoted as $M$). 
% It is the time span from the emerging of the first item till the finish of the last task. 
% We set the emerging time of the first item to be $0$ w.l.o.g and then $M$ is equal to the finish time of the last rack returned (as in \eqref{eq:makespan}).
% \begin{equation}
% \label{eq:makespan}
%     M = \max_{r \in R} f_r
% \end{equation}
% where $f_r$ denotes the latest time at which rack $r$ is returned.
% It can be calculated as below.
% \begin{equation} 
% \label{eq:finishRack}
% \begin{aligned}
%     f_r = & t_k + d(l_a, l_r) + d(l_r, l_{p_r}) + \max\{d(l_a, l_r) + d(l_r, l_{p_r}) - f_p,  0\} \\
%     & + \sum_{i\in \tau_r}i + d(l_{p_r}, l_r)
% \end{aligned}
% \end{equation}
% where $t_k$ is the last time the rack being selected.
% Following five terms are corresponding to time consumption of five step.
% $d(\cdot, \cdot)$ denotes path length between two locations given by the planning algorithm.
% By assuming the robot moving at unit velocity, its value is equal to time consumption.
% $f_p$ is the finish time of picker $p$ to finish all items of all racks in queue.
% It can be calculated as \equref{eq:finishPicker}, and the max term in \equref{eq:finishRack} denotes queuing time.
% \begin{equation}
% \label{eq:finishPicker}
%     f_p = e_p + \sum_{r \in q_p} \sum_{i \in \tau_r} i
% \end{equation}

%We will introduce our solution with high adaptability (\secref{sec:selection}) to overcome the first challenge and efficiency design (\secref{sec:efficient}) for the second one.

% \fakeparagraph{Remarks}
% Solving this problem is confronted with two challenges.
% \begin{itemize}
%     \item \emph{Online setting.} To overcome this challenge, the algorithm should considers spatio temporal status of racks and the pickers due to the complex coupling, which requires for high adaptability.
%     \item \emph{Internal planning complexity.} As for this challenge, though prior works \cite{AAAI21LJY, AAMAS17Ma} have studied conflict-free path finding problem, we notice that the growing logistic demands poses large-scale issue for the scheduling, thus potential scalability support is indispensable.
% \end{itemize}
% We will introduce our solution with high adaptability (\secref{sec:selection}) to overcome the first challenge and efficiency design (\secref{sec:efficient}) for the second one.

%Then two sub process approximation and bootstrap are described in \secref{subsec:greedy} and \secref{subsec:qlearning}, respectively.

% In our settings, we have three options for agent: picker, robot and rack.
% Since one picker are responsible for multiple racks, modeling each picker as an agent may suffer with too large granularity.
% As for the choice between robot and rack, based on the intuitive explanations in \secref{subsec:greedy}, rack and picker have more dynamic temporal status thus require more consideration than robot, so we set rack as agent.

Rack selection in warehouse has been studied recent years \cite{EJOR17Boysen, IJPR17Zou}.
However, \cite{IJPR17Zou} depends on queuing-theoretic model deriving strong assumptions to handle the highly dynamic property, making these solutions hard to extend to rack-to-picker mode.
\cite{EJOR17Boysen} studies minimizing the number of moving racks when one order may be composed on items from several racks.
This study relies on linear programming and it suffers scalability issue when confronted with large scale throughput.
In fact, this problem has not been studied sufficiently due to its internal complexity \cite{EJOR07De}.

As for the traversal process, building an index to support nearest search seems feasible, but the highly dynamic of robots making the index design itself becomes a question.
For the second bottleneck, the conflict-free constraint makes it hard for acceleration.
We will introduce our acceleration next section.

However, compared with the second bottleneck in planning, this acceleration is still not enough.
Next two subsections describe optimizations on the second bottleneck.

Though large discrepancy may exist between the optimal solution and greedy, we find that using that as an approximation is enough for the learning process.

    \item \emph{Planning path for each assigned robot.}
    The path planning process requires A* search.
    To avoid conflict, the search takes place in a spatio temporal graph.
    The spatio temporal correlated property increase the searching space, leading to both time consuming and space consuming.

\fakeparagraph{Token Passing}
TP is one of the most classical algorithm to MAPF problem\cite{AAMAS17Ma}.
It finds conflict-free paths in a decentralized manner.
A token is passing among all AMRs and the one who get the passing try to find its closest task and search a path via A* algorithm.

\fakeparagraph{Rolling-Horizon Collision Resolution (RHCR)}
RHCR is proposed by \cite{AAAI21LJY}, whose basic idea is to planning via A* algorithm only for some steps (window), and after some steps it will planning again.

\fakeparagraph{Bottleneck Matching (BM)}
This method tries to maximize the matching cardinality while minimizing the maximum picker's finishing time after picking.

However, the above successful applications of reinforcement learning-based methods inspire us some potential trials on seamlessly integrating spatio temporal data mining and decision making.


\subsection{Moving object and indoor space management}
As RFID and Wi-Fi based positioning technologies emerged, a large amount of indoor spatial temporal data is available, which enables researches on indoor space data management and mining. 
The main challenge of indoor spatial temporal data management is mainly about two aspects\cite{DEB10Jensen}. \textit{(i)} unlike outdoor positioning technique such as GPS, indoor space positioning technologies are not precise or continuous. \textit{(ii)} Indoor spaces contains doors, walls, aisles forming a topological space rather than Euclidean spaces as outdoor.
Surmounting the first challenge requires to comprehensively use multi source of indoor positioning data \cite{MDM09Becker, MDM11Baniukevic}. 
To overcome the second challenge calls for new design of index.
\cite{ICDE12Lu} and \cite{VLDB16Shao} propose graph-based and tree-based models for indoor spaces to support spatial queries, respectively.
Recently, due to the outbreak of COVID-19, crowd-aware query attracts some interests of indoor research community\cite{VLDB21Liu}. 
Some other relevant work \cite{TKDE18Li} devise a data-driven approach for searching the dense indoor region.

Though our automatic rack-to-picker scenario happens at indoor spaces, it is quite different from prior studies.
First, robots moving schemes are programmed and do not face the uncertainty of traditional moving objects.
Second, robots can be precisely positioned and manipulate to given locations via the technology of robot control.
Third, a warehouse layout is much simpler than indoor venues such as shopping mall or office.
However, the unique challenges of this problem has not been sufficiently studied in indoor research community.

Rack selection in warehouse has been studied recent years \cite{EJOR17Boysen, IJPR17Zou}.
However, \cite{IJPR17Zou} depends on queuing-theoretic model deriving strong assumptions to handle the highly dynamic property, making these solutions hard to extend to rack-to-picker mode.
\cite{EJOR17Boysen} studies minimizing the number of moving racks when one order may be composed on items from several racks.
This study relies on linear programming and it suffers scalability issue when confronted with large scale throughput.
In fact, this problem has not been studied sufficiently due to its internal complexity \cite{EJOR07De}.

However, task selection has been studied extensively in spatiotemporal crowdsourcing scenario.
\cite{GEO16Deng} studies select tasks from worker's perspective to maximize the number of finished tasks.
However, it studies a static scenario that all tasks are known at first.
\cite{GIS20Camila} studies to minimize worker's detour when he or she is fulfilling a spatio task while new tasks may emerge and he or she can fulfill them in-route.
This problem is interesting but our robot can only carry one rack and their solution degrades to simple shortest path finding.

More popularly, spatiotemporal crowdsourcing research community will integrate the task selection and allocation to work and directly study the task assignment problems \cite{VLDB20Tong, ICDE16Tong, KDD18Xu, KDD21Tang}.
Task assignment has been viewed as the core issue of spatio temporal crowdsourcing, a killer app in mobile Internet era \cite{VLDB20Tong}.
It is usually modeled as a bipartite matching problem, where vertices from two sides represented tasks and workers respectively.
To capture the dynamic property, prior works usually adopt online setting, \ie tasks arrives in a streaming manner.
\cite{ICDE16Tong} further extended into a dynamic setting, where both workers and tasks arrives dynamically.
Though many assignment algorithms proposed after years studies, many of them can hardly beat the most naive greedy algorithm\cite{VLDB16Tong}.
This may because pure combinatorial algorithms fail to mine the spatio temporal data pattern for better assignment decisions.
For better understanding the patterns from spatio temporal data, \cite{KDD17Tong} propose a linear model with over 100 million features to predict the future demands.
The prediction will help for better assignment decisions.
Instead of predicting and making assignment decision separately, reinforcement learning based method can integrates two phases together.
\cite{KDD18Xu} proposes to model the sequential assignment decisions as Markov decision process and use dynamic programming to mining historical spatio temporal data for assignment decision.
\cite{KDD21Tang} and \cite{KDD21Shi} further extends it to an online manner which can mining from spatio temporal data and making assignment decisions simultaneously.

These methods can not be trivially extended into our settings, mainly because our complex spatio temporal coupling among racks, robots and pickers.

Though path planning has also been studied in spatio temporal crowdsourcing \cite{VLDB18Tong, ICDE10Hans, ICDE14Bin, VLDB20Zeng, SIGMOD15She, SIGSPATIAL15Li}, these studies is not suitable in our multiple robots scenario.



% \begin{figure*}
% \centering
% 	\subfigure[Normal]{
% 		\includegraphics[width=0.23\linewidth]{fig/normal_M.pdf}
% 		\label{fig:normalM}
% 	}
% 	\subfigure[Large]{
% 		\includegraphics[width=0.23\linewidth]{fig/large_M.pdf}
% 		\label{fig:largeM}
% 	}
% 	\subfigure[Real]{
% 		\includegraphics[width=0.23\linewidth]{fig/real_M.pdf}
% 		\label{fig:realM}
% 	}
% 	\subfigure[Super Large]{
% 		\includegraphics[width=0.23\linewidth]{fig/superLarge_M.pdf}
% 		\label{fig:superLargeM}
% 	}
% 	\caption{Makespan comparison over all datasets.}
% 	\label{fig:makespan}
% \end{figure*}

% Rack selection in warehouse has been studied recent years \cite{EJOR17Boysen, IJPR17Zou}.
% However, \cite{IJPR17Zou} depends on queuing-theoretic model deriving strong assumptions to handle the highly dynamic property, making these solutions hard to extend to rack-to-picker mode.
% \cite{EJOR17Boysen} studies minimizing the number of moving racks when one order may be composed on items from several racks.
% This study relies on linear programming and it suffers scalability issue when confronted with large scale throughput.
% In fact, this problem has not been studied sufficiently due to its internal complexity \cite{EJOR07De}.
% \TODO{why put them here?}



% Reinforcement learning \cite{sutton2018reinforcement} finds a policy for agents who interact with an environment.
% Agent is modeled as state and the interactions with environment (\ie actions) are expressed as state transitions.
% Each transition associates with a reward sent from the environment.
% The policy is derived from a value function, which maps the state and its transition to the expected accumulative rewards.
% The policy chooses the transition which maximizes the expected accumulative rewards, while the state implies information about the environment and agent.

% Reinforcement learning is fit for sequential decision making problems with the Markov property.
% Here we sequentially make decisions on whether to select a rack for transport and processing.
% The problem also has Markov property because we make decisions for the current timestamp only considering the current situation rather than history.

%For adaptive and efficient learning of planning decisions, we consider online bootstrap learning such as q-learning \cite{watkins1989}.

% \dy{
% Our reward design considers not only the time usage of processing but that of delivery as well, which makes our algorithm be planning-aware.
% Intuitively, if the corresponding picker's $ap_r$ is large, the max term will be mainly depended on it rather than the delivery time usage (\ie $d(l_r, l_{p_r})$), thus the distance between rack and picker will not be considered as a critical factor.}

\begin{algorithm}[t]
\label{alg:cacheSearch}
    \caption{Cache-Aided Search}
	\Input{$v_s$: source vertex, $v_d$: destination, $L$: distance threshold}
	\Output{$u$: path from $v_s$ to $v_d$ without conflict with current paths}
	\textbf{Initialize} \\
	$Cache \leftarrow \emptyset$ \\ 
    \For{$g_s \leftarrow $ \text{ all grid vertex}}{
        \For{$g_t \leftarrow$ \text{whose distance to }$g_s \le L$ }{
            $u' \leftarrow \text{ find shortest path via BFS }$ \\
            $Cache  \leftarrow Cache \cup \{\langle g_s, g_t\rangle : u'\}$
        }
    }
	\textbf{Planning} \\ 
	$Q \leftarrow \emptyset$ \\
	$\text{Add } v_s \text{ in } Q$ \\
	\While{$Q \text{ is not empty }$}{
	    $v_c \leftarrow \text{ vertex with the least h-value in } Q$ \\
	    $u' \leftarrow \text{try to get from } Cache $ \\
	    \If{$u' \ne \text{NULL}$}{
	        $u \leftarrow \text{derive by waiting till no conflict happens}$ \\
	        \textbf{break} \\
	    }
	    \For{$v_a \leftarrow \text{ adjacent to } v_c$}{
	        \If{$v_a \text{ is not visited and } v_a \text{ bears no conflict}$}{
	            $\text{set h-value of } v_a \text{ as } d(v_c) + 1 + dist(v_a, v_d)$ \\
	            $\text{set prior of } v_a \text{ as } v_c$ \\
	            $\text{Update h-value and prior of } v_a \text{ to } Q$ \\
	        }
	    }
	}
	$u \leftarrow \text{ derive the path via backtracking the prior}$ \\
	\Return{$u$}
\end{algorithm}

Line 8 to 21 are the query stage which searches for the path from the given source and the destination without conflict.
In summary, our cache-aided search follows the framework of the A* algorithm except that in line 12 to 15 it tries to use the cache to derive the path directly.
Then it will use cache-aided search to plan paths for each selected rack (line 7 to 11).
All planed paths will be inserted to the conflict detection index for further conflict avoidance (line 12) and the update operation will be executed periodically to control its memory usage (line 5 to 6).


% Our optimization goal is to minimize $M$.
% To achieve this, we are required to design a rack selection algorithm $\mathcal{A}$ which considers temporal status of both racks and their corresponding pickers' temporal statuses and output a selection scheme $S = \{r_1, r_2, ...\}$ at each time unit.
% All schemes $\{S_1, S_2, ..., S_k\}$ should be \emph{sufficient} to fulfill all items emerged.


%Intuitively, a good rack selection scheme will balance the workload of pickers and use robot wisely to avoid robot shortage when large amount of racks are requiring delivery.
%Though rack selection is the critical factor to the picking system efficiency.
%We still need a planning algorithm for the following fulfillment process. 

%Specifically, it requires assigning an idling robot for each selected rack and planning paths for them.

% So for each selection scheme, a corresponding planning scheme $U$ is generated which contains a set of paths (\ie spatio-temporal coordinates) $\{\langle t_1, x_1, y_1\rangle, \langle t_2, x_2, y_2, \rangle ...\}$.
% The planning scheme should satisfy following constraints.
% \begin{itemize}
%     \item \emph{feasibility constraints.} The robot $a$ to be assigned should be available (\ie $s_a$ is idling).
%     \item \emph{Conflict-free constraints.} All paths should avoid \emph{same visit} conflict and \emph{head on} conflict.
% \end{itemize}

% The definitions of above two types of conflicts are as below.
% \begin{itemize}
%     \item \emph{Same visit.} For any two paths, visiting the same location at the same time is not allowed (See \figref{fig:expSV}).
%     \item \emph{Head on.} For any two paths $u_1$ and $u_2$ in all planning schemes, there should not exist $\langle t_i, x_i, y_i \rangle, \langle t_{i + 1}, x_{i+1}, y_{i+1} \rangle$ in $u_1$ and $\langle t_j, x_j, y_j \rangle, \langle t_{j + 1}, x_{j + 1}, y_{j + 1} \rangle$ in $u_2$ such that $t_i=t_{j+1} \land t_{i+1} = t_j \land x_i=x_{j+1} \land y_i = y_{j+1} \land x_{i+1}=x_j \land y_{i+1} = y_j$ (See \figref{fig:expHO}).
% \end{itemize}

==> body/trash_intro.tex <==
% \TODO{to discuss:
% 1. What is the base problem? \eg online task assignment? multi-agent path finding?
% 2. Better justify the motivation in terms of scalability and dynamics.
% 3. Why reinforcement learning is not used in previous studies?
% 4. Is indoor space important?}
Boosting of E-commerce releases large amount of logistic demands.
During last year's online shopping carnival in China, over 2 billion logistic orders (worth over 115 billion dollars) are created\footnote{https://www.cnbc.com/2020/11/12/singles-day-2020-alibaba-and-jd-rack-up-record-115-billion-of-sales.html}.
The large amount of logistic orders poses large-scale throughput challenge to warehouses which store and distribute goods to buyers.
Million-scale daily throughput workload calls for revolution of warehouse \cite{IR16Robert}.
Though robotic techniques provide basis for improving the performance via robots \cite{AI08Wurman}, the spatio-temporal related scheduling of robots is the key to enhance the performance\cite{IJPR17Ren}.

In an automatic warehouse, the mostly adopted rack-to-picker scenario contains five steps to fulfill an order.
Specifically, when an online shopping order (\ie a task requiring delivering and picking) emerged, we need to choose an idle robot and planing a path for it to \textit{(i)} pick up the rack where the order's item is located, and \textit{(ii)} the robot deliver the rack to its corresponding picker,\textit{(iii)} wait to be picked and \textit{(iv)} after finish picking it will \textit{(v)} return the rack via the planed paths.
A good scheduling strategy, composed of assignment and collision-free path planning will reduce the makespan of all tasks and thus improve the throughput of the warehouse.

Traditional spatio temporal task assignment or multi-agent path finding methods, however, are not capable of the current large-scale and highly automatic warehouse mainly because of the following reasons.
\begin{itemize}
    \item \emph{Complex spatio-temporal coupling for task assignment.}
    Unlike traditional spatio temporal task assignment which has mainly been studied in crowdsourcing\cite{VLDB20Tong, ICDE19Wang},
    fulfilling a task requires cooperation between pickers and robots.
    Each picker's responsibility for multiple racks from different locations, causing delivered tasks queuing for picking, which leads to a spatio-temporal coupling causing intractability of optimization. 
    \item \emph{Large-scale requirements for path planning.} 
    Traditional path planning methods such as \cite{AI13Sharon, AI15Sharon, AAMAS17Ma} propose search-based methods aiming to find collision-free paths for multiple robots, however, those search-based methods suffers scalability issue and there validation scales are no more than 1000 tasks.
    In our settings, however, daily process requirement can be up to million tasks, far more larger than their settings.
\end{itemize}

In this paper, we first formulate the automatic rack-to-picker scenario as Robot-Task Assignment and path Planning (RTAP) problem.
We analysis the hardness and find that naive greedy method does not have a constant competitive ratio.
Then we propose a spatio-temporal system called Assignment and Planning Service (\sysname).
It contains both a coupling-aware task assignment algorithm and an efficient multi robots path planning algorithm.
When tasks are coming, the task assignment algorithm will get and evaluate the current temporal state of pickers and racks to decides which tasks will be delivered, then it assigns those tasks to the robots.
After that, the path planning algorithm calculate collision-free paths for robots and send the schemes to robots to execute.

The task assignment algorithm use reinforcement learning model to capture the temporal properties of pickers and tasks based on historical data.
This data-driven approach enables task assignment algorithm with high adaptability.
The route planning algorithms are designed based on widely applied A* algorithm.
To cope with the large-scale issue, a grid-based index is designed and upon it we devise a dynamic programming based cache for acceleration.

To the best of our knowledge, our work is the first to consider both task assignment and path planning in such warehouse systems, unlike prior studies relating to multi-agent path finding.
Besides, we stress on practical issue by conducting test on large-scale and real datasets.
Our contributions can be summarized as follows.
\begin{itemize}
    \item We formulate the Robot Task Assignment and path Planing problem (RTAP), which captures the properties of robots, tasks and pickers.
    We also theoretically analysis the hardness of this problem.
    \item We propose a reinforcement learning based assignment method which shows a powerful adaptability for the complex spatio temporal coupling.
    \item An index is designed and a dynamic programming aided routing algorithm is proposed for efficient conflict-aware path planning.
    \item We conduct experiments on both synthesized and real datasets, the results validate the performance.
\end{itemize}

The rest of this paper are organized as follows.
In \secref{sec:problem} we formulate the problem and analyze its hardness, then we introduce the framework of our \sysname system.
The task assignment algorithm and path planning algorithm are introduced in \secref{sec:selection} and \secref{subsec:efficent}, respectively.
We evaluate our method in \secref{sec:evaluation} and present the related work in \secref{sec:related}.

% However, merely depending on robotic techniques is not enough to maintain the operation of a part-to-picker systems.
% Besides, a continuously functioning part-to-picker system requires
% This Multi-Agent Path Finding problem (MAPF) has attracted large research interests\cite{AI13Sharon, AI15Sharon, IJCAI15Boyarski, AAAI13Yu, AAAI21LJY}.
% These researches provide solutions for conflict-free requirement, which enables feasibility and reliability of modern AMR-driven warehouse.
%During the last ten years, the boost of E-commerce releases large deliver demand and raises challenges relating to large-scale and highly dynamic order emergence, which calls for higher efficiency requirement\cite{IR16Robert}.
% The task assignment between AMRs and picking task decides the orders' batching, picking and routing, which are all critical to the efficiency of warehouse\cite{IJPR17Ren}.
%Though task assignment in the large-scale and dynamic spatio-temporal scenario has been studied in crowdsourcing\cite{VLDB16Tong, ICDE16Tong, ICDE19Wang, ICDE17Song, ICDE18Zeng},
% these methods cannot be trivially extended into this setting due to the following reasons. 

% \begin{itemize}
%     \item \emph{Multiple-stage temporal dependency.} 
%     Each picker is responsible of multiple racks but he or she can only pick one task of a certain rack at a time, causing other delivered racks queuing.
%     This waiting process causing a strong dependency among tasks.
%     What's worse, the AMR cannot be released when queuing (since it needs to return the rack), which weakens the shipment ability of AMRs.
%     \item \emph{Efficient conflict-aware indoor routing.} 
%     Unlike the task assignment in spatio-temporal crowdsourcing, the worker are usually assumed to route by itself.
%     But AMRs are not capable of self-routing, especially under conflict-free constraints.
%     Though prior studies relating to MAPF provide some methods, some efficient design are required for the large-scale scenario. 
% \end{itemize}

% \begin{itemize}
%     \item \emph{Limitation 1: Lack scalability.} Some traditional search such as \cite{AI13Sharon, AI15Sharon, IJCAI15Boyarski} search on the whole feasible solution space aiming to find the optimal solution, while some other A* based searching algorithms \cite{AAAI13Yu, AAAI21LJY} trading accuracy for efficiency.
%     However, all the above algorithms suffers scalability issue, their experiments contains no more than 1000 picking tasks.
%     \item \emph{Limitation 2: Lack dynamic description.} 
%     Most of the current researches focus on one shot optimization \cite{AI13Sharon, AI15Sharon, IJCAI15Boyarski}, \ie all AMRs and picking tasks are static.
%     Though there are some recent studies consider a life-long scenario \cite{AAMAS17Ma, AAAI21LJY}, where tasks are arriving following streaming manner, but they lack the consideration of dynamics of picker, \ie the picking time for each task.
%     The picking time will cause the AMR queuing for picking which may change the bottleneck and thus dwarf these solutions performances.
% \end{itemize}

% \begin{itemize}
%     \item \emph{Spatio resources are scarce.} 
%     The aisles in warehouse is usually narrow to maximize the number of racks.
%     The scarce  spatio resources leading to high probability of collisions.
%     Planning conflict-free routes is a must for all AMRs in those narrow warehouse aisles.
%     \item \emph{Temporal dependencies are complex.}

%     \item \emph{Spatio-temporal correlation is critical to the whole efficiency.}
%     The assignment results decides how to planning routes for each AMR while the routes' lengths reversely decides the temporal states.
%     In fact, this problem is a mixture of assignment and planning, and a cooperative design will help improve the system performance.
% \end{itemize}

% Though dynamic large-scale task assignment and route planning at indoor spaces has been studied in data engineering community \cite{VLDB16Tong, ICDE16Tong, VLDB00Pfoser, SIGMODL00Simonas, DEB10Jensen, ICDE12Lu}.
% Studies aiming at spatio temporal task assignment has capture the dynamic description from one side online to the two-sided dynamic scenario\cite{VLDB20Tong}.
% These model are suitable for crowdsourcing but are not trivial to extend to the assignment between AMRs and racks, due to the dynamic of pickers.
% Other studies aiming at moving object and indoor spaces though provide good query and management for trajectories and indoor spaces, the conflict-free constraints limit the extension of their methods.

% The above reasons call for new design capturing the multiple-stage temporal dependency and new routing query algorithm satisfying both conflict and efficient requirement.
% In this paper, we first analysis the problem.
% The theoretical analyzing result shows that naive method does not have a constant approximate ratio and the bad cases reveal how the multiple-stage dependency amplifies the impacts of spatio-temporal dynamics on the naive method's performance.
% Based on the above observations, we design a reinforcement learning based assignment algorithm.
% To capture the temporal dependency property, we segment the picking time of pickers and racks as state, and to overcome the bootstrap issue, we integrate the naive greedy method as approximation together with q-learning for better evaluation. 
% We also embed the wide adopt $\epsilon$-greedy policy into for our efficient design.
% To overcome the large-scale indoor routing issue, we design conflict detect index.
% The index records all prior planned trajectories and supports for quick detection for conflicts.
% Based on the index, we design an A* based route planning algorithm, which has been widely used for robot routing.
% To accelerate the query process, we use dynamic programming policy and pre-compute and record short paths without considering conflict.
% These pre-recored paths helps largely reduces the open set size in A* algorithm thus making the query process suitable for the large-scale scenario.
